Learning Multi-Agent Loco-Manipulation for Long-Horizon Quadrupedal Pushing

Recently, quadrupedal locomotion has achieved significant success, but their manipulation capabilities, particularly in handling large objects, remain limited, restricting their usefulness in demanding real-world applications such as search and rescue, construction, industrial automation, and room organization. This paper tackles the task of obstacle-aware, long-horizon pushing by multiple quadrupedal robots. We propose a hierarchical multi-agent reinforcement learning framework with three levels of control. The high-level controller integrates an RRT planner and a centralized adaptive policy to generate subgoals, while the mid-level controller uses a decentralized goal-conditioned policy to guide the robots toward these sub-goals. A pre-trained low-level locomotion policy executes the movement commands. We evaluate our method against several baselines in simulation, demonstrating significant improvements over baseline approaches, with 36.0% higher success rates and 24.5% reduction in completion time than the best baseline. Our framework successfully enables long-horizon, obstacle-aware manipulation tasks like Push-Cuboid and Push-T on Go1 robots in the real world.

==> contents/experiments_icra_submission.tex <==
% To validate our proposed method, we implement extensive experiments in both simulation and on the physical robots.
% in this section, extensive numerical simulations and hardware experiments are presented. Numerical simulations are performed in the IsaacGym environment as a high-fidelity physics engine \cite{makoviychuk2021isaac}.
% Simulation and experiment videos are available in the supplementary material.

\subsection{Simulation Setups}
\subsubsection{Environments and Tasks}\label{subsubsec:env and task}
We build our simulation environments in IsaacGym \cite{makoviychuk2021isaac}.
We consider a cluttered environment with randomly placed \(1.0\,\text{m} \times 1.0\,\text{m}\) obstacles, where multiple quadrupeds need to push a target object to a desired goal. Unitree Go1 robots are utilized in simulation to match the physical robots, each with an approximate payload capacity of 5 kg. 
% The friction coefficient on the ground is randomly assigned between 0.4 and 0.6, while the target objects have a constant friction coefficient of 0.5. 
The robots are tested with three types of objects varying
in shape and mass: a 4 kg cube (\(1.2\,\text{m} \times 1.2\,\text{m})\), a 3 kg T-shaped block, and a 10 kg cylinder with a radius of 1.5 m.
Different numbers of agents are evaluated across tasks, with two agents for the cube and T-shaped block, and up-to four agents for the cylinder.
% Different numbers of agents are evaluated across different tasks (2\,for\,cube\&T, 3\,for\,cylinder). 
The initial positions and postures of the agents and target objects are randomly set within a small range on one side of the room, while the target goals for the object are generated on the other side. The task is considered successful if the center of the object is positioned within 1 m of the target. Failure occurs in the situation described in Sec. \ref{subsubsec:high-level reward} . The tasks are designed for challenging long-horizon pushing, with initial-to-target distances exceeding 10 m. 
% Additional details can be found in the Appendix.

\subsubsection{Baselines}
% We introduce the following three baselines to evaluate the effectiveness of our proposed method.
We compare our proposed method with the following baselines.

\textbf{Single-Agent (SA)} retains the three hierarchical levels of the policy and the reward function design, but only a single quadrupedal robot is employed for each task.

\textbf{High-Level+Low-Level (H+L)} utilizes both a high-level and a low-level policy, where the high-level policy proposes subgoals for the robots, and the low-level policy aids the robots in navigating to these subgoals. We maintain $r^h_{\text{task}}$ and $r^h_{\text{penalty}}$ mentioned in Sec. \ref{subsubsec:high-level reward}. This baseline follows a similar approach to \cite{nachum2019multi}, with a multi-agent implementation using MAPPO \cite{yu2022surprising}.

\textbf{Mid-Level+Low-Level (M+L)} retains the mid-level and low-level policies without using a high-level policy to provide subgoals, meaning the robots are guided directly by the distant final target. 
% $r^m_{\text{task}}$ and $r^m_{\text{penalty}}$.
Similar to the methods proposed in \cite{xiong2024mqe} and \cite{an2024solving}, we maintain $r^m_{\text{task}}$ and $r^m_{\text{penalty}}$ mentioned in Sec. \ref{subsubsec:mid-level reward}. In addition, extra heuristic rewards, $r^m_{\text{approach}}$ and $r^m_{\text{vel}}$, are added to promote the long-horizon pushing performance of the mid-level network. 
% This baseline also serves as a multi-agent extension of \cite{jeon2023learning}.

\subsection{Simulation Results and Analysis}
\subsubsection{Comparisons with Baselines}\label{sec:main_result}
Training was carried out in 500 environments, accumulating 60 million steps, each 10 million steps taking approximately one hour of simulation time. The performance of each method is summarized in Table \ref{tab:main_result}. The success rate (S.R.) is evaluated over 50 trials, averaging results from four random seeds with a frozen low-level policy. The completion time (C.T.) represents the average time taken by the robots to complete the pushing task in 50 trials. If a failure occurs during the task, the completion time is recorded as the timeout duration.

\begin{table}[htp]
\vspace{-8pt}
\scriptsize
\centering
\caption{Success rates and completion time ($\pm$ standard deviation) of our method and baselines in different settings in simulation. The completion time is scaled to $[0,1]$ where $1$ means taking up a full episode reaching the timeout.}
\label{tab:main_result}
\begin{tabular}{cc|cccc}
\toprule
\multicolumn{2}{c|}{Task}                    & SA           & H+L             & M+L            & \textbf{Ours}           \\
\midrule
\multirow{2}{*}{Cube}     & S.R.$\uparrow$ & 4.5$\pm$0.3\%    & 0.23$\pm$0.02\% & 18.1$\pm$8.0\% & \textbf{77.5$\pm$3.0\%} \\
                          & C.T.$\downarrow$ & 0.98$\pm$0.02  & 1.00$\pm$0.00   & 0.88$\pm$0.05  & \textbf{0.66$\pm$0.04}  \\
\midrule
\multirow{2}{*}{T-Shape}  & S.R.$\uparrow$   & 21.2$\pm$9.3\% & 9.0$\pm$6.0\%   & 18.8$\pm$8.6\%  & \textbf{63.5$\pm$7.7\%} \\
                          & C.T.$\downarrow$ & 0.96$\pm$0.04  & 0.94$\pm$0.04   & 0.86$\pm$0.06  & \textbf{0.68$\pm$0.04}  \\
\midrule
\multirow{2}{*}{Cylinder} & S.R.$\uparrow$ & 0.0$\pm$0.0\%  & 3.0$\pm$4.0\%   & 31.0$\pm$24.5\%  & \textbf{71.2$\pm$5.1\%} \\
                          & C.T.$\downarrow$ & 1.00$\pm$0.00  & 0.99$\pm$0.02   & 0.82$\pm$0.16  & \textbf{0.48$\pm$0.01}  \\ 
\bottomrule
\end{tabular}
\vspace{-12pt}
\end{table}


%\begin{table}[htp]
%\tiny
%\centering
%\caption{Success rates and completion time of the proposed method and baselines in different settings in simulation}
%\label{tab:main_result}
%\begin{tabular}{ccccccc}
%\toprule
%\multirow{2}{*}{Method} & \multicolumn{2}{c}{Cube} & \multicolumn{2}{c}{T} & \multicolumn{2}{c}{Cylinder} \\
%\cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7}
%& \multicolumn{1}{c}{S.R.$\uparrow$} & \multicolumn{1}{c}{C.T.$\downarrow$} & \multicolumn{1}{c}{S.R.$\uparrow$} & \multicolumn{1}{c}{C.T.$\downarrow$} & \multicolumn{1}{c}{S.R.$\uparrow$} & \multicolumn{1}{c}{C.T.$\downarrow$} \\
%\midrule
%S.R.            & 4.5$\pm$0.3\%           &     0.98$\pm$0.02      & 21.2$\pm$9.3\%          & 0.96$\pm$0.04          & 0.0$\pm$0.0\%           & 1.00$\pm$0.00  \\
%H+L             & 0.23$\pm$0.02\%         &     1.00$\pm$0.00      & 9.0$\pm$6.0\%           & 0.94$\pm$0.04          & 3.0$\pm$4.0\%           & 0.99$\pm$0.02  \\
%M+L             & 10.5$\pm$8.5\%          &     0.95$\pm$0.04      & 1.8$\pm$1.0\%           & 0.99$\pm$0.01          & 3.0$\pm$3.0\%           & 0.80$\pm$0.02  \\
%\textbf{Ours}   & \textbf{77.5$\pm$3.0\%} &\textbf{0.66$\pm$0.04}  & \textbf{63.5$\pm$7.7\%} & \textbf{0.68$\pm$0.04} & \textbf{71.2$\pm$5.1\%} & \textbf{0.48$\pm$0.01}   \\
%\bottomrule
%\end{tabular}
%\end{table}

As shown in Table \ref{tab:main_result}, the proposed method achieves an average success rate exceeding 60\% in all tasks involving three distinct objects. In contrast, the \textbf{Single-Agent} method exhibits a success rate below 25\%, as a single robot lacks sufficient strength needed for effective pushing, underscoring the importance of multi-robot coordination. The \textbf{H+L} method also faces challenges, with a similarly low success rate. In some situations, the object movements towards the final goal are disrupted by the other one or two agents, even if the agents can usually reach their own subgoals.
This highlights the difficulty of aligning agent-wise subgoals with effective push control, particularly given the complexity of object interactions, indicating the need for a more fine-grained coordination. 
The \textbf{M+L} method outperforms \textbf{H+L} by enabling more elaborate collaboration, but it exhibits greater variability across different seeds. 
Likewise, it still struggles with the long-horizon nature of the task, as its higher-level policy has difficulty effectively guiding the object towards the distant target.

\begin{table}[htp]
\vspace{-9pt}
\centering
\caption{The results of the OCB-reward ablation study. Two methods are evaluated under two timeout conditions. }
\label{tab:ocb_ablation}
\begin{tabular}{cccccc}                         
\toprule
                                                              & \multicolumn{2}{c}{Timeout=20s} & \multicolumn{2}{c}{Timeout=40s} \\
\cmidrule(lr){2-3} \cmidrule(lr){4-5}
\multicolumn{1}{l}{}                                          & S.R.$\uparrow$         & C.T.$\downarrow$            & S.R.$\uparrow$          & C.T.$\downarrow$    \\         
\midrule
\textbf{Ours}                                                 & \textbf{57.0$\pm$6.1\%}        & \textbf{14.9$\pm$0.8}        & \textbf{74.0$\pm$6.9\%}        & \textbf{22.5$\pm$2.4}     \\   
Ours w/o OCB  & 13.0$\pm$1.2\%                                        & 18.3$\pm$0.2        & 19.0$\pm$2.6\%        & 34.9$\pm$0.3        \\
\bottomrule
\end{tabular}
\vspace{-8pt}
\end{table}
% \vspace{-12pt}


\subsubsection{Ablation Study}
\paragraph{The OCB Reward}
To assess the effectiveness of the OCB reward in training the mid-level controller for short-horzion pushing, we conduct an ablation study in a free space environment, where a 6 kg cube (\(1.5\,\text{m} \times 1.5\,\text{m})\) is placed with random orientations. Two agents are randomly initialized, while the target object position (subgoal for the mid-level controller) is generated within a circular area 1.5 to 3.0 m from the cube's initial position randomly. 
% Success was defined as moving the cube within 1.0 m of the target point, with time limits set at 20 and 40 s.
As shown in Table \ref{tab:ocb_ablation}, our method significantly outperforms the ablation experiment in both success rate (S.R.) and completion time (C.T.). In particular, as the duration of the timeout increases, the success rate of our method improves more rapidly, indicating a better adaptability to adjust the direction of pushing when the object deviates, an issue that often causes failures with shorter timeouts.

\begin{figure}[H]
    \centering
    \begin{subfigure}[b]{0.23\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/Avoid1.pdf}
        \caption{Ours w/o adaptive policy.}
        \label{subfig:adaptive/RRT}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.23\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/Avoid.pdf}
        \caption{Ours.}
        \label{subfig:adaptive/ours}
    \end{subfigure}
    \label{fig:adaptive}
    \caption{Comparison between our method and the one with only the RRT planner at the high-level controller.}
\vspace{-6pt}
\end{figure}

\paragraph{The High-Level Adaptive Policy}
To demonstrate the need for an adaptive high-level controller, we design a challenging scenario with obstacles placed directly between the start and target positions of the T-block. Although the RRT planning algorithm finds a short path, it often leads to trajectories that come too close to obstacles without considering the object shape, failing to account for the dynamics of the pushing process and lacking real-time adjustments based on the object's state (Fig. \ref{subfig:adaptive/RRT})
In contrast, our method deviates from obstacles in advance, allowing the robots to bypass them and reach the goal (Fig. \ref{subfig:adaptive/ours}), underscoring the importance of the RL-trained high-level adaptive policy.

\begin{figure}[H]
    \centering
    \includegraphics[width=0.90\linewidth]{figures/SR.pdf}
    \caption{The success rate and completion time of different numbers of robots in the task of cylinder pushing.}
    \label{fig:scalibility_result}
    \vspace{-8pt}
\end{figure}

\begin{figure*}[h]
    \centering
    \includegraphics[width=0.95\textwidth]{figures/real_world_experiment_v6.pdf} 
    \caption{The \textcolor{blue}{blue part} demonstrates the effect of pushing the T-shaped block in the real environment, while the \textcolor{red}{red part} illustrates the cube-pushing results in the real environment. In each section, the top-left figure shows the movement trajectories of the robots and the object. The bottom-left figure displays the angular velocity commands received by the robots. The top-right figure shows the linear velocity commands received by robot 1, and the bottom-right figure shows the linear velocity commands received by robot 2. The middle part contains screenshots of the video corresponding to the completion of each task. We have extracted key frames that align well with the 2D trajectories, providing a clear visual comparison.}
    \label{fig:real_world_experiment}
    \vspace{-12pt}
\end{figure*}

\subsubsection{Scalability Analysis}
To evaluate the scalability of the proposed method, we experiment with different numbers of robots to push the cylinder described in Sec. \ref{subsubsec:env and task}. As shown in Fig. \ref{fig:scalibility_result}, both the success rate and the completion time improve significantly as the number of robots increases. However, once the number of robots reaches four, the success rate decreases compared to that with three robots. This decline could be due to an increased risk of collisions, which causes robots to maintain greater distances from each other, which leads to less coordinated behaviors.



\subsection{Real-World Setups}
\subsubsection{Environments and Task}
We evaluate our policy on real hardware in a 7.5 m $\times$ 7.5 m room, utilizing two Unitree Go1 robots, each with an approximate payload of 5 kg. The entire room is equipped with 24 Primex 22 cameras, using OptiTrack's motion capture system to gather real-time data regarding robots and objects. We deploy both our high-level and low-level policies, trained in simulation, on physical robots, utilizing the integrated locomotion policy of the Unitree Go1 as the low-level controller for real-world experiments. With domain randomization implemented for the higher-level policy and the low-level policy trained with Real-to-Sim considerations outlined in Section \ref{sec:low-level}, we observe that this zero-shot transfer demonstrates robustness.

% Since we have utilized the domain randomization when training our policies in simulation, we try to directly deploy the mid-level and high-level networks trained in simulation on the real robots. However, we use a different low-level controller. The WTW policy employed in simulation is found to exhibit significant discrepancies between the commanded and actual speeds when deployed on the real robots; notably, different units demonstrate varying degrees of deviation, resulting in a substantial Sim2Real gap. Nevertheless, we find that Unitree's high-level controller can accurately execute corresponding commands while maintaining compatibility with the command format used by our low-level controller during simulation. Therefore, we ultimately adopt Unitree's high-level controller as the low-level controller. However, since Unitree's high-level controller does not provide open-source code for parallel training in simulation, we choose to unified parameters of the low-level controller in simulation, such as gait and body height, with those of the Unitree high-level controller. This ensures that the low-level controllers in both the simulation and the real robot are almost identical.

We conduct two tasks for two robots: pushing a cube and pushing a T-shaped block. The cube utilized in the experiment measures $1.5\,\text{m} \times 1.0\,\text{m}$ and weighs 6.8 kg. The T-block consists of a main body measuring $0.5\,\text{m} \times 1.0\,\text{m}$, with a protruding section measuring $0.5\,\text{m} \times 0.5\,\text{m}$, and has an overall weight of 3.3 kg. 
Specifically, in the cube task, the target position is randomly set on the opposite side of the room, constrained within an $x$-range of 5.5 m to 6.5 m and a $y$-range of -3.5 m to 3.5 m. In the T-pushing task, the target position is set within an $x$-range of 3.5 m to 4.5 m and a $y$-range of -4 m to 4 m,. Even with a limited size of the physical environment, this setup ensures that our pushing process remain sufficiently long to meet the requirements of long-horizon tasks. Additionally, in the cube-pushing task, obstacles are randomly initialized within a narrow 2 m band surrounding the line connecting the starting and target positions of the box.

\subsection{Real-World Results and Analysis}

\subsubsection{Pushing T}
As shown in the blue part of Figure~\ref{fig:real_world_experiment}, the robots effectively control the turning of the T-shaped block, and successfully push the T-block to the target position. Due to the smaller size of the T-shaped block, finding the appropriate pushing point is crucial for the task. We observe that the two robots consistently push from the two ends of the block to apply a larger contact surface, which ensures the application of continuous forward force while also maintaining directional control. 
% This result is consistent with the strategy we observe in simulation.

Additionally, we find that the $x$ direction velocity commands output by the mid-level policy almost always reach the upper bound of 0.5. It is reasonable because once the robots identify the correct pushing points, the pushing action is primarily forward, with turning achieved by adjusting their own yaw. Since the target is located in the positive $y$ direction, we observe that the yaw command is initially positive and gradually returns to zero or negative after the turn is completed to straighten the robots. This is complemented by minor $y$ direction velocity commands, which help adjust the robots' positions, aligning well with our expectations.

\subsubsection{Pushing Cube}

% The push-cube task is challenging due to the large size and weight of the cube, is a typical multi-robot collaboration task. Since this task involves a longer pushing distance with obstacles, it further tests the planning and coordination capabilities between different layers of our hierarchical framework in real world. As shown in the red part of Figure~\ref{fig:real_world_experiment}, the robots push the box along an adaptive trajectory that successfully avoids the obstacles and reaches the target. 
% The large volume of the cube also provides a substantial contact surface, offering sufficient contact points. We observe that the two robots adopt different pushing postures at various stages of the task to achieve different effects. Sometimes, both robots push forward with their heads to maintain maximum forward speed, while at other times, one or both robots push sideways to facilitate turning. This behavior is consistent with the results we observe in the simulation. Similarly, we find that the $x$-direction velocity commands output by the policy almost always reach the upper bound of 0.5, for the same reasons as the push-T task. Since there is no significant turning in this pushing process, the $y$-direction commands and yaw rate commands constantly adjust, which also aligns with our expectations.

The push-cube task, a typical multi-robot collaboration challenge, is difficult due to the cube's large size and weight. It involves long-distance pushing with obstacles, testing the planning and coordination of our hierarchical framework. As shown in Figure~\ref{fig:real_world_experiment}, the robots push the box along an adaptive trajectory, avoiding obstacles and reaching the target. The cube’s large surface offers ample contact points, allowing the robots to adopt different pushing postures as needed. At times, both push forward for speed, while at others, they push sideways to turn, consistent with our simulation results. The $x$-direction velocity commands often hit the 0.5 upper bound, similar to the push-T task, while $y$-direction and yaw rate commands adjust as expected due to minimal turning.

\vspace{-3pt}


==> contents/methodology_icra_submission.tex <==
\begin{figure}[htp]
    \centering
    \includegraphics[width=\linewidth]{figures/framework.pdf}
    \caption{The framework of our proposed hierarchical MARL method for quadrupedal pushing.}
    \label{fig:framework}
\end{figure}
\vspace{-8pt}

\subsection{Hierarchical Reinforcement Learning for Long-Horizon Multi-Robot Pushing}
To enable quadrupedal robots to collaboratively perform long-horizon pushing tasks in environments with obstacles, we propose a hierarchical reinforcement learning framework, as illustrated in Figure \ref{fig:framework}.  
This framework consists of three layers of controllers. At the top level, an RRT planner generates a geometrically feasible trajectory without accounting for the robots' pushing capabilities or the dynamics of multiple robots and the object. 
% \textcolor{blue}{The RRT planner helps agents find reasonable paths in any complex environment, avoiding the huge exploration and learning cost of adapting to new cluttered scenarios.} 
The high-level adaptive policy then uses this trajectory as a reference to assign a subgoal for the target object, based on the dynamic states of the environment, object, and robots.
Using this common subgoal, each robot's mid-level pushing policy provides velocity commands to its corresponding low-level policy.
% The mid-level polices of all robots are trained collaboratively using multi-agent reinforcement learning, while it is executed in a decentralized manner. The low-level locomotion policy will generate target joint positions for the PD controller on the robot to track.
% The mid-level policies of all robots are collaboratively trained using MARL but executed in a decentralized manner. At the lowest level, the locomotion policy generates target joint positions for the robot's PD controller to follow.
% Due to the computation time of the RRT planner, it is only implemented once at the start of the episode. Both the high-level adaptive policy and the mid-level controller has a frequency of 50Hz, and we find it beneficial to use a higher frequency at the higher level for more adaptive policy in our settings. The low-level locomotion policy has a frequency of 50Hz. The PD controller in simulation is implemented at 200Hz while on the robot it is at 2000Hz.
Due to the computational demands of the RRT planner, it is executed only once at the start of each episode. Both the high-level adaptive policy and the mid-level controller operate at a frequency of 50 Hz, with the higher frequency at the high level proving beneficial for more adaptive behavior in our settings. The low-level locomotion policy also runs at 50 Hz, while the PD controller is implemented at 200 Hz in simulation and 2000 Hz on the physical robot.
In the following sections, we will introduce each of these three hierarchies in detail.

\subsection{Low-Level Controller}
\label{sec:low-level}

The low-level controller controls each robot individually to track the mid-level velocity commands.
More specifically, each low-level controller $\pi^{l,i}_{\varphi}: \mathcal{O}^{l,i}\rightarrow\mathcal{A}^{l,i}$ computes motor commands $a^{l,i}$ to track the mid-level velocity command $a^{m,i}=(v^i_{x}, v^i_{y}, v^i_{\text{yaw}})$.
Despite recent progress of learning-based low-level controllers \cite{margolis2023walk}, we find these controllers to suffer from a large sim-to-real gap, and cannot accurately track the velocity commands, especially when the robot is pushing a heavy object.
Instead, we use Unitree's built-in low-level controller, which tracks the velocity commands significantly more robustly in the real world.
For efficient policy training in simulation, we train a learned low-level policy to mimic the behavior of Unitree's built-in controller.

We create the simulated low-level controller based on \emph{Walk-These-Ways} (WTW) \cite{margolis2023walk}.
As an RL framework for low-level motor control, WTW can learn locomotion behaviors with configurable body pose, gait timing, and reference velocity.
We measure these parameters on the built-in controller, and reproduce them in WTW to learn similar behaviors.
During upper-level policy training, we invoke the low-level WTW policy in parallel on GPU, which significantly reduced the training time.

% The low-level controller $\pi^{l,i}_{\varphi}: \mathcal{O}^{l,i}\rightarrow\mathcal{A}^{l,i}$ is a decentralized locomotion policy of agent $i$, where $\mathcal{O}^{l,i}$ represents the low-level local observation space of robot $i$, and $A^{l,i}$ is the action space of the mid-level policy of agent $i$. $\pi^{l,i}_{\varphi}$ takes the local observation of agent $i$, $o^{l,i}\in\mathcal{O}^{l,i}$, and the linear velocity and yaw rate commands, $a^{m,i}=(v^i_{x}, v^i_{y}, v^i_{\text{yaw}})$, from the mid-level controller as the input, and output a low-level action, $a^{l,i}\sim\pi^{l,i}_{\phi}(a^{l,i}|o^{l,i},a^{m,i})\in\mathcal{A}^{l,i}$, which are desired joint positions of quadrupedal robot $i$. The torque of each joint will be computed via a PD controller to track the desired joint position.

% We follow the training scheme
% , including the reward, domain randomization, and curriculum settings
% of \textit{Walk-These-Ways} (WTW) \cite{margolis2023walk} to train our low-level locomotion policy for all agents in simulation. In practice, we find that the WTW policy has a large Sim-to-Real gap and cannot track velocity commands accurately and robustly, especially when in contact with the object, and the gap can vary largely across different robots. Meanwhile, we find that the integrated locomotion policy (IP) of the Unitree Go1 is robust for pushing objects. Therefore, we follow a Real-to-Sim procedure for WTW policy training in simulation, during which we set the command sampling range centered around the measured locomotion parameters of the IP, including the gait timing offsets, body roll, body pitch, body height, and foot swing height. When the lower-level policy is employed by the upper-level policy training, we set the commands to track the measured IP parameters to make it aligned with the locomotion policy on physical robots.

\subsection{Mid-Level Controller}
The mid-level controller $\pi^{m,i}_{\phi}: \mathcal{O}^{m,i}\rightarrow\mathcal{A}^{m,i}$ is a decentralized policy of agent $i$, where $\mathcal{O}^{m,i}$ represents the mid-level local observation space of robot $i$, and $A^{m,i}$ is the action space of the mid-level policy of agent $i$. This decentralized policy takes as input the high-level action $a^{h}$, the local observation of robot $i$, $o^{m,i}\in\mathcal{O}^{m,i}$, which consists of the local observations of the target object state $s^i_{\text{object}}$, obstacle state $s^i_{\text{obstacle}}$, and the state of other robots, $\{s^i_{j}\}^N_{j=1,j\neq i}$, all computed in the local torso frame of the robot $i$. For example, $s^i_{\text{object}}$ can be expanded as $(x^i_{\text{object}}, y^i_{\text{object}}, \psi^{i}_{\text{object}})$, where $(x^i_{\text{object}}, y^i_{\text{object}})$ is the 2D position of the object, and $\psi_{\text{object}}$ is its yaw angle, both in the local frame of robot $i$. The mid-level policy of agent $i$ will output a mid-level action $a^{m,i}\sim\pi^{m,i}_{\phi}(a^{m,i}|o^{m,i},a^h)\in\mathcal{A}^{m,i}$ in a decentralized manner
% which can be expanded by $a^{m,i}=(v^i_{x}, v^i_{y}, v^i_{\text{yaw}})$, which are linear and yaw rate commands 
to the low-level controller of robot $i$. 

In practice, we train a mid-level policy shared by all robots, noted as $\pi^m_{\phi}$.
Following the scheme of centralized training and decentralized execution, it is trained by MAPPO \cite{yu2022surprising} to optimize the objective function $\mathcal{J}^m(\theta)=\mathbb{E}_{\tau\sim\rho_\pi}\left[\sum_{t=0}^T{\gamma^tr^m(s_t, a^h_{t}, \{a^{m,i}_t\}^N_{i=1})}\right]$, where $s_t$ is a joint state at time $t$, $\tau$ is the trajectory sampled from a distribution $\rho_\pi$ induced by policy $\pi^m_{\phi}$, initial state $\rho^m_0$ and the transition probability $p^m$ that are defined by the mid-level task. Here, $r^m(\cdot)$ represents the reward function for the mid-level controller. During training, we randomly sample the subgoals of the object as $a^h$ and freeze the low-level policy. Meanwhile, we specialize the domain randomization for frictions to reduce the Sim2Real gap of pushing.

\subsection{High-Level Controller}
The high-level controller is composed of two elements, a RRT planner $\mathcal{P}:\mathcal{M}\times\mathcal{G}\rightarrow \mathcal{T}$ and a centralized adaptive policy $\pi^{h}_{\theta}:\mathcal{M}\times\mathcal{T}\times \mathcal{S}_{\text{object}}\times \mathcal{S}_1\times \mathcal{S}_2\times \cdots \mathcal{S}_N\rightarrow \mathcal{A}^h$, where $\mathcal{M}$ represents the map information space, $\mathcal{G}$ represents the goal space of the target object, $T$ represents the trajectory space of the RRT planner, $\mathcal{S}_{\text{object}}$ denotes the object state space, $\mathcal{S}^i$ is the state space of robot $i$, and $A^h$ is the action space of the high-level adaptive policy.

The RRT planner takes the desired goal position of the object $g_{\text{object}}\in\mathcal{G}$ and the map information $p_{\text{map}}\in\mathcal{M}$ encompassing the obstacle position and the initial position of the object as input and outputs a reference trajectory $\tau_r\in\mathcal{T}$ for the adaptive policy $\pi^h_{\theta}$. The adaptive policy will use the desired goal $g_{\text{object}}$, each robot state $s_i\in \mathcal{S}_i$, the map information $p_{\text{map}}$ and the dynamic global object pose $s_{\text{object}}\in \mathcal{S}_{\text{object}}$, as the input, and output a high-level action $a^h\sim \pi^h_{\theta}(a^h|g_{\text{object}}, p_{\text{map}}, s_1, s_2, \cdots, s_N, s_{\text{object}}, \tau_r)\in\mathcal{A}^h$ as the subgoal position of the target object to the mid-level policy $\pi^m_{\phi}$.
The high-level adaptive policy is a centralized policy and trained via PPO \cite{schulman2017proximal} to optimize the objective function $\mathcal{J}^h(\theta)=\mathbb{E}_{\tau\sim\rho_\pi}\left[\sum_{t=0}^T{\gamma^tr^h(g_{\text{object},t}, p_{\text{map},t}, s_{\text{object},t}, \{s_{i,t}\}^N_{i=1},a^h_t, \tau_r)}\right]$ , where $\tau$ is the trajectory sampled from a distribution $\rho_\pi$ induced by policy $\pi^h_{\theta}$, initial state $\rho^h_0$ and the transition probability $p^h$ that are defined by the high-level task, Here, $r^h(\cdot)$ represents the reward function for the high-level controller. During training, we freeze the mid-level and low-level controller.

% \vspace{-6pt}

\subsection{Reward Design}
\label{subsec:reward}
\subsubsection{High-Level Reward} 
\label{high-level reward}
\label{subsubsec:high-level reward}
The high-level reward function is composed of two terms: \(r^h = r^h_{\text{task}} + r^h_{\text{penalty}}\). The high-level task reward \(r^h_{\text{task}}\) provides a sparse reward for reaching the final target and two dense rewards: one for minimizing the distance between the subgoal and the nearest point on the RRT trajectory, and the other for reducing the distance between the object and the final target. This guides the robots to follow the RRT trajectory while allowing minor deviations for handling push complexities.

The high-level penalty \(r^h_{\text{penalty}}\) includes penalties for close distances to obstacles and severe punishments for exceptions such as robot falls, collisions, object shaking, and timeouts.

\subsubsection{Mid-Level Reward}
\label{subsubsec:mid-level reward}
Our mid-level reward function is formulated as $r^m = r^m_{\text{task}} + r^m_{\text{penalty}} + r^m_{\text{heuristic}}$. Similar to high-level reward, the mid-level task reward $r^m_{\text{task}}$ rewards actions for approaching and reaching the target point, and the mid-level penalty $r^m_{\text{penalty}}$ punishes close distances among agents, as well as exception situations described in Sec. \ref{high-level reward}. 

Additionally, the mid-level heuristic reward \(r^m_{\text{heuristic}} = r^m_{\text{approach}} + r^m_{\text{vel}} + r^m_{\text{OCB}}\). The mid-level approaching reward \(r^m_{\text{approach}}\) encourages agents to approach the object, while the velocity reward \(r^m_{\text{vel}}\) is awarded when the object's velocity exceeds a set threshold, promoting various pushing actions and preventing oscillation near the object.

In addition, we also introduce an occlusion-based reward \(r^m_{\text{OCB}}\) inspired by \cite{chen2015occlusion}, designed to guide agents toward more favorable contact points. To compute \(r^m_{\text{OCB}}\), we first determine the nearest point on the convex hull of the object relative to the position of the agent. Next, we calculate the dot product between the normal vector at this point and the target direction. Agents are rewarded or penalized based on this dot product, which is critical in pushing tasks where identifying optimal contact points is challenging. This reward encourages agents to target occluded surfaces, enabling more effective pushing behavior.

In particular, \(r^m_{\text{heuristic}}\) plays a crucial role in the push process, given the large action space and the inherent uncertainty and complexity of interactions during push.
